A study of the Gribov-Zwanziger action: from propagators to glueballs

This Ph.D. thesis presents a study of the Gribov-Zwanziger framework: from propagators to glueballs. The chapters 2 and 3 are meant as an introduction and only require a basic knowledge of quantum field theory. Chapter 2 explains the techniques behind algebraic renormalization, which shall be widely used throughout this thesis, while chapter 3 tries to give a pedagogic overview of the Gribov-Zwanziger framework as this is not available yet in the literature. The subsequent chapters contain own research. First in chapter 4, we shall dig a bit deeper in the Gribov-Zwanziger framework, by exploring the BRST symmetry and the KO criterium. Next, in chapter 5 we shall elaborate on the ghost and the gluon propagator in the infrared and present a refined Gribov-Zwanziger action. Further, we present two chapters on the search for physical operators within the (refined) Gribov-Zwanziger framework, chapter 6 and 7. A small chapter 8 is devoted to some values for different glueballs. We end this thesis with the conclusions, chapter 9.

==> conclusie.tex <==
\chapter*{Conclusie}
\addcontentsline{toc}{chapter}{Conclusie}
Hier komt de conclusie


==> overview.tex <==
\chapter{Introduction}
\section*{Introduction}
Quantum Chromodynamics (QCD) is the theory which describes the strong interaction, one of the four fundamental forces in our universe. This force describes the interactions between quarks and gluons, which are fundamental building blocks of our universe. At very high energies, QCD is asymptotically free, meaning that quarks and gluons should be freely detected. However at low energies, i.e~our daily world, due to the strong force, quarks and gluons interact and form bound states called hadrons. A well known example of these bound states are the proton and the neutron, but a whole zoo of hadrons has been observed in particle detectors. In fact, the only way to obtain information about the strong force is through bound states, as no free quark or gluon has even been detected. We call this phenomenon \textit{confinement}. Although since the formulation of the standard model (which includes QCD), 40 years of intensive research have past, no good answer has been found to probably one the most fundamental questions in QCD. Even the formulation of what confinement really is, is under discussion.\\
 \\
The difficulty for solving confinement lies in the fact that the standard techniques which have been so successful in QED, are not applicable in QCD. In QED the coupling constant is small enough\footnote{This depends of course on the energy range of interest.}, so one can apply perturbation theory, which amounts to writing down a series in the coupling constant. With every next term of the series, one can converge more to the exact answer. As in QCD, the coupling constant increases for decreasing energies, the coupling constant is much to high and perturbation theory alone can never give a good description of the theory. Therefore, other techniques are required which we call non-perturbative methods. There exists a wide range of non-perturbative methods, which all try to approach QCD from one way or another. One should not see these different techniques as competing, but as patchwork trying to cover all aspects of QCD.\\
\\
Even if one omits quarks in QCD, one can still call the remaining theory confining. Although there is no real experimental evidence, lattice simulations have shown that gluons form bound states which we call glueballs and no free gluon shall be detected. Therefore, it is already interesting to investigate pure QCD without quarks, and try to find out what happens. One could say that confinement is hidden in the behavior of the gluons.\\
\\
As all fundamental forces, QCD is gauge theory and the pure gluonic part can be described by the $SU(N)$ Yang-Mills action for $N=3$. In QCD we call $N$ the color, as $N=3$ QCD has three different colors, usually presented as red, green and blue.\\
\\
In this thesis, we shall also work around confinement. For simplicity, we shall omit quarks and work with pure Yang-Mills theory. We shall also try to cover one part of the patchwork. \\
\\



\section*{Organization of the thesis}
The thesis is organized as follows. The first two chapters are introductions. I


Part I \\
-First introduction on algebraic renormalization \\
-Then the gribov problem explained + GZ action\\
(hier ook kondo paper in verwerken)\\
Part II research\\
- introduction on lattice\\
- relation between KO en GZ \\
- Refined GZ action 4D \\
- Refined GZ action 3D \\
- Refined GZ action 2D \\
Part III the quest for physical operators\\
-$F^2$ in glueballs in YM\\
-$F^2$ in GZ\\
- i particles

